Fully-Automated Verification of Linear Systems Using Inner- and Outer-Approximations of Reachable Sets

Reachability analysis is a formal method to guarantee safety of dynamical systems under the influence of uncertainties. A substantial bottleneck of all reachability algorithms is the necessity to adequately tune specific algorithm parameters, such as the time step size, which requires expert knowledge. In this work, we solve this issue with a fully automated reachability algorithm that tunes all algorithm parameters internally such that the reachable set enclosure respects a user-defined approximation error bound in terms of the Hausdorff distance to the exact reachable set. Moreover, this bound can be used to extract an inner-approximation of the reachable set from the outer-approximation using the Minkowski difference. Finally, we propose a novel verification algorithm that automatically refines the accuracy of the outer-approximation and inner-approximation until specifications given by time-varying safe and unsafe sets can be verified or falsified. The numerical evaluation demonstrates that our verification algorithm successfully verifies or falsifies benchmarks from different domains without requiring manual tuning.

==> subtex/oldstuff.tex <==

% --- error constant input solution in IV-A.1)

%Let us first consider the error contained in the particular solution $\overPu{t_k}$ due to constant inputs.
%
%\begin{proposition} (Error constant input solution) \label{prop:eaccu}
%The Hausdorff distance between the exact constant input solution
%%
%\begin{equation*}
%	\Pu{t_{k+1}} = \int_{0}^{t_{k+1}} e^{A(t_{k+1} - \theta)} \mathrm{d}\theta \, \uTrans{}
%\end{equation*}
%%
%and the outer-approximation
%%
%\begin{equation*}
%	\overPu{t_{k+1}} = \overPu{t_k} \oplus e^{At_k} \overPu{\Delta t_k} ,
%\end{equation*}
%%
%with $\overPu{\Delta t_k} = \zono{\widehat{c}_p^{\prime},\widehat{G}_p^{\prime}}$ computed in \lineref{alg:standard:overPu_k} in \algref{alg:standard}, is bounded by
%%
%\begin{equation} \label{eq:eaccu}
%	\eaccu{k+1} = \eaccu{k} + \eaccustep{k} ,
%\end{equation}
%%
%where the error $\eaccustep{k}$ for one time step is
%%
%\begin{equation} \label{eq:eaccustep}
%	\eaccustep{k} := 2 \errOp{ \zono{ \matzeros{}, e^{At_k} \widehat{G}_p^{\prime} } } .
%\end{equation}
%\end{proposition}
%%
%\begin{proof}
%Since the exact constant input solution is just a single point, the error $\eaccustep{k}$ is given by the size of the entire additional set $e^{At_k} \overPu{\Delta t_k}$ (see \eqref{eq:eaccustep}).
%The propagation formula in \eqref{eq:eaccprop} then directly yields the accumulation in \eqref{eq:eaccu}.
%\end{proof}

% --- error constant input solution in IV-A.1)




% --- error affine solution with overPu in IV-A.1)

%\begin{proposition} (Error affine dynamics) \label{prop:eps_affine}
%Consider the sets $\HPtp{t_k} = \zono{c_h,G_h}$, $\overPu{t_k} = \zono{\widehat{c}_p,\widehat{G}_p}$, and $\overPu{\Delta t_k} = \zono{\widehat{c}_p^{\prime},\widehat{G}_p^{\prime}}$, where $G_h \in \R{n \times \gens{}_h}$, $\widehat{G}_p \in \R{n \times \widehat{\gens{}}_p}$, and $\widehat{G}_p^{\prime} \in \R{n \times \widehat{\gens{}}_p^{\prime}}$.
%The Hausdorff distance between the exact time-interval solution of the affine dynamics
%%
%\begin{align*}
%	\HPti{\tau_k} &= \big\{ e^{At} x(t_k) + A^{-1}(e^{A (t - t_k)} - I) \uTrans{} ~ \big| \\
%		&\qquad \quad t \in \tau_k, x(t_k) \in \HPtp{t_k} \big\}
%\end{align*}
%%
%and the corresponding outer-approximation
%%
%\begin{equation} \label{eq:overHPti}
%	\overHPti{\tau_k} = \linCombOp{\overHPtp{t_k}, \overHPtp{t_{k+1}}} \oplus \C{} \\
%\end{equation}
%%
%in \lineref{alg:standard:overHPti_k} of \algref{alg:standard} is bounded by
%%
%\begin{equation} \label{eq:eps_affine}
%	\dH{\HPti{\tau_k},\overHPti{\tau_k}} \leq \ehom{k} + \eaccu{k+1} ,
%\end{equation}
%%
%with $\eaccu{k+1}$ as in \propref{prop:eaccu} and
%% 	\eaccu{k+1} &:= 2 \errOp{ \zono{ \matzeros{}, \tilde{G}_p } } , \label{eq:eaccu}
%%	where $\tilde{G}_p$ is the generator matrix of $\overPu{t_{k+1}}$ and
%\begin{align}
%	\ehom{k} &:= \ecomb{k} + \eC{k} , \label{eq:ehom} \\
%	\ecomb{k} &:= \sqrt{\gens{}_h + \widehat{\gens{}}_p + \widehat{\gens{}}_p^{\prime}} \,
%		\norm{[G_h^{(-)}~\widehat{G}_p^{(-)}~\widehat{G}_p^{\prime}]}_2 , \label{eq:ecomb} \\
%	\eC{k} &:= 2 \errOp{ \C{} } , \label{eq:eC}
%\end{align}
%%
%where $G^{(-)}_h := (e^{A\Delta t_k} - I) G_h$, $\widehat{G}^{(-)}_p := (e^{A\Delta t_k} - I) \widehat{G}_p$.
%\end{proposition}
%%
%\begin{proof}
%\rmk{possibly subject to change...}
%On a high level, one first requires to measure the error induced by the linear combination for zonotopes \eqref{eq:ecomb}, which itself contains the set $\overPu{t_k}$ and thus its accumulated error \eqref{eq:eaccu}.
%The error \eqref{eq:eC} results from the enlargement of the linear combination.
%The remaining details can be found in \appref{app:eps_affine}.
%\end{proof}

% --- error affine solution with overPu in IV-A.1)




% --- proof error affine solution with overPu in appendix

%Zonotopes are not closed under linear combination \eqref{eq:zonoLinComb}, which requires us to measure the induced error by
%%
%\begin{equation} \label{eq:dHcomb}
%	\dH{ \linCombOp{\HPtp{t_k},\HPtp{t_{k+1}}}, \linCombOpZ{\overHPtp{t_k},\overHPtp{t_{k+1}}} } ,
%\end{equation}
%%
%where we use $\linCombOpZ{\cdot}$ to explicitly denote the over-approximation of the linear combination for zonotopes \eqref{eq:zonoLinComb}.
%To compute \eqref{eq:dHcomb}, we first define the shorthand notation
%%
%\begin{align*}
%	\S{} &= \linCombOp{\HPtp{t_k},\HPtp{t_{k+1}}} , \\
%	\Sover{} &= \linCombOp{\overHPtp{t_k},\overHPtp{t_{k+1}}} , \\
%	\Zover{} &= \linCombOpZ{\overHPtp{t_k},\overHPtp{t_{k+1}}} ,
%\end{align*}
%%
%and apply the triangle inequality to \eqref{eq:dHcomb}, yielding
%%
%\begin{equation} \label{eq:dHcombtriangle}
%	\dH{ \S{}, \Zover{}} \leq \dH{\S{}, \Sover{}} + \dH{\Sover{}, \Zover{}} .
%\end{equation}
%%
%To evaluate both terms on the right-hand side, we introduce the following sets
%%
%\begin{alignat}{2}
%	&\HPtp{t_k} = \zono{c_h, G_h}, \qquad												&& G_h \in \R{n \times \gens{}_h}, \label{eq:def_HP} \\
%%	&\overHPtp{t_k} = \zono{\widehat{c}_h,\widehat{G}_h}, \qquad						&& \widehat{G}_h \in \R{n \times \widehat{\gens{}}_h}, \label{eq:def_overHP} \\
%	&\Pu{\Delta t_k} = \zono{c_p^{\prime},[~]},											&& ~ \label{eq:def_Pu_init} \\
%	&\overPu{\Delta t_k} = \zono{\widehat{c}_p^{\prime},\widehat{G}_p^{\prime}}, \qquad	&& \widehat{G}_p' \in \R{n \times \widehat{\gens{}}_p^{\prime}}, \label{eq:def_overPu_init} \\
%	&\Pu{t_k} = \zono{c_p,[~]}, \qquad													&& ~ \label{eq:def_Pu_k} \\
%	&\overPu{t_k} = \zono{\widehat{c}_p,\widehat{G}_p}, \qquad							&& \widehat{G}_p \in \R{n \times \widehat{\gens{}}_p}. \label{eq:def_overPu_k}
%\end{alignat}
%
%\begin{lemma} \label{lmm:eps_affine_2}
%The Hausdorff distance between the exact and over-approximative linear combination of the exact affine solutions can be bounded by \eqref{eq:eaccu}, i.e.,
%%
%\begin{equation*}
%	\dH{\S{}, \Sover{}} \leq 2 \errOp{ \zono{ \matzeros{}, \tilde{G}_p } } ,
%\end{equation*}
%%
%where $\tilde{G}_p$ is the generator matrix of $\overPu{t_{k+1}}$.
%\end{lemma}
%\begin{proof}
%%
%Inserting into the definition \eqref{eq:dH}, we obtain
%%
%\begin{equation} \label{eq:S_Sover}
%	\dH{ \S{}, \Sover{} } = \max_{\widehat{s} \in \Sover{}} \min_{s \in \S{}} \norm{\widehat{s} - s}_2
%\end{equation}
%%\begin{align}
%%	&\dH{ \S{}, \Sover{} } = \max \Big\{ \max_{s \in \S{}}
%%		\big( \, \min_{\widehat{s} \in \Sover{}} \, \norm{\widehat{s} - s}_2 \, \big),
%%		\max_{\widehat{s} \in \Sover{}} \big( \, \min_{s \in \S{}} \norm{\widehat{s} - s}_2 \, \big) \Big\} \nonumber \\
%%	&\quad = \max_{\widehat{s} \in \Sover{}} \min_{s \in \S{}} \norm{\widehat{s} - s}_2 \label{eq:S_Sover}
%%\end{align}
%%
%due to the containment $\S{} \subseteq \Sover{}$ which follows from $\HPtp{t_k} \subseteq \overHPtp{t_k}$ and the definition of the linear combination \eqref{eq:defLinComb}.
%To express the linear combinations $\S{}$ and $\Sover{}$, we adapt \lineref{alg:standard:overHPtp_k} by reordering of matrices and sets to obtain an equivalent propagation formula:
%%
%\begin{align*}
%	\HPtp{t_{k+1}} &= e^{A t_{k+1}} \initset{} + \Pu{t_{k+1}} \\
%		&= e^{A \Delta t_k} \underbrace{(e^{A t_k} \initset{} + \Pu{t_k})}_{=\,\HPtp{t_k}} + \Pu{\Delta t_k}, \\
%	\overHPtp{t_{k+1}} &= e^{A \Delta t_k} \overHPtp{t_k} \oplus \overPu{\Delta t_k}. 
%\end{align*}
%%
%Now, we insert \eqref{eq:def_HP}-\eqref{eq:def_overPu_k} into $\S{}$ and $\Sover{}$:
%%
%\begin{align*}
%	\S{} &= \bigg\{ \lambda \big(c_h + \sum_{i=1}^{\gens{}_h} G_{h(\cdot,i)} \varphi_i + c_p \big)
%		+ (1-\lambda) \big( e^{A\Delta t_k} \cdot \\
%	&\;\; (c_h + \sum_{i=1}^{\gens{}_h} G_{h(\cdot,i)} \varphi_i + c_p) + c_p' \big)
%		~ \bigg| ~ \varphi_i \in [-1,1], \lambda \in [0,1] \bigg\} , \\
%	\Sover{} &= \bigg\{ \lambda \big( c_h + \sum_{i=1}^{\gens{}_h} G_{h(\cdot,i)} \varphi_i
%		+ \widehat{c}_p + \sum_{i=1}^{\widehat{\gens{}}_p} \widehat{G}_{p(\cdot,i)} \chi_i \big) \\
%	&\;\; + (1-\lambda) \big( e^{A\Delta t_k} (c_h + \sum_{i=1}^{\gens{}_h} G_{h(\cdot,i)} \varphi_i
%		+ \widehat{c}_p + \sum_{i=1}^{\widehat{\gens{}}_p} \widehat{G}_{p(\cdot,i)} \chi_i) \\
%	&\;\; + \widehat{c}_p^{\prime} + \sum_{i=1}^{\widehat{\gens{}}_p^{\prime}} \widehat{G}_{p(\cdot,i)}^{\prime} \chi_i^{\prime} \big)
%	~ \bigg| ~ \varphi_i, \chi_i, \chi_i^{\prime} \in [-1,1], \lambda \in [0,1] \bigg\} .
%\end{align*}
%%
%We yield an upper bound for the minimum in \eqref{eq:S_Sover} by equating the respective $\lambda$ and $\varphi_i$ in $\S{}$ and $\Sover{}$ and thus
%%
%% \lVert and \rVert_2 instead of norm{}_2 because it does not span over multiple lines
%\begin{align*}
%	&\max_{\widehat{s} \in \Sover{}} \min_{s \in \S{}} \norm{\widehat{s} - s}_2 \\
%	&\qquad \leq \max_{\substack{\chi_i \in [-1,1] \\ \chi_i^{\prime} \in [-1,1] \\ \lambda \in [0,1]} }
%		\big\lVert \lambda \big( \widehat{c}_p + \sum_{i=1}^{\widehat{\gens{}}_p} \widehat{G}_{p(\cdot,i)} \chi_i - c_p \big) \\
%	&\qquad \qquad + (1-\lambda) \big( e^{A\Delta t_k}( \widehat{c}_p + \sum_{i=1}^{\widehat{\gens{}}_p} \widehat{G}_{p(\cdot,i)} \chi_i - c_p ) \\
%	&\qquad \qquad + \widehat{c}_p^{\prime} + \sum_{i=1}^{\widehat{\gens{}}_p^{\prime}} \widehat{G}_{p(\cdot,i)}^{\prime} \chi_i^{\prime} - c_p^{\prime} \big) \big\rVert_2 ,
%\end{align*}
%%
%which takes on its maximum at the boundary $\lambda \in \{0,1\}$ for any choice of $\chi_i, \chi_i^{\prime} \in [-1,1]$.
%For the two cases, we have
%%
%\begin{alignat*}{3}
%	&\lambda = 0: \;	&& \Pu{t_k} \subset \overPu{t_k} \; \Rightarrow \; \norm{\widehat{c}_p - c_p}_2 \leq \errOp{\zono{\matzeros{},\widehat{G}_p}} , \\
%	&\lambda = 1: \;	&& e^{A \Delta t_k} \Pu{t_k} + \Pu{\Delta t_k} \subset e^{A \Delta t_k} \overPu{t_k} \oplus \overPu{\Delta t_k} \\
%	&~					&& \Rightarrow \; \norm{ e^{A \Delta t_k} \widehat{c}_p + \widehat{c}_p^{\prime} - (e^{A \Delta t_k} c_p + c_p^{\prime}) }_2 \\
%	&~					&& \qquad \quad \leq \errOp{\zono{\matzeros{},[e^{A \Delta t_k}\widehat{G}_p~\widehat{G}_p^{\prime}]}} .
%\end{alignat*}
%%
%Thus, we apply \lmmref{lmm:dH_2err} in both cases, which yields
%%
%\begin{align*}
%	&\max_{\chi_i \in [-1,1]} \big\lVert \widehat{c}_p - c_p + \sum_{i=1}^{\widehat{\gens{}}_p} \widehat{G}_{p(\cdot,i)} \chi_i \big\rVert_2 \leq 2 \errOp{\zono{\matzeros{},\widehat{G}_p}} , \\
%	&\max_{\substack{\chi_i \in [-1,1] \\ \chi_i^{\prime} \in [-1,1] }} \big\lVert e^{A\Delta t_k} \widehat{c}_p + \widehat{c}_p^{\prime} - (e^{A\Delta t_k} c_p + c_p^{\prime}) \\
%	&\qquad \qquad + e^{A \Delta t_k} \sum_{i=1}^{\widehat{\gens{}}_p^{\prime}} \widehat{G}_{p(\cdot,i)}^{\prime} \chi_i^{\prime} + \sum_{i=1}^{\widehat{\gens{}}_p} \widehat{G}_{p(\cdot,i)} \chi_i \big\rVert_2 \\
%	&\quad \leq 2 \errOp{\zono{\matzeros{},[e^{A \Delta t_k}\widehat{G}_p~\widehat{G}_p^{\prime}]}}
%\end{align*}
%%
%and finally,
%%
%\begin{equation} \label{eq:dH_S_Sover}
%	\max_{\widehat{s} \in \Sover{}} \min_{s \in \S{}} \norm{\widehat{s} - s}_2
%	\leq 2 \errOp{ \zono{ \matzeros{}, [e^{A \Delta t_k}\widehat{G}_p~\widehat{G}_p^{\prime}] } } ,
%\end{equation}
%%
%as $\widehat{G}_p$ and $[e^{A \Delta t_k}\widehat{G}_p~\widehat{G}_p^{\prime}]$ are the generator matrices of $\overPu{t_k}$ and $\overPu{t_{k+1}}$, respectively, and $\overPu{t_{k+1}} \supset \overPu{t_k}$ by the propagation formula in \lineref{alg:standard:overPU_k} in \algref{alg:standard}.
%\end{proof}
%
%\begin{lemma} \label{lmm:eps_affine_3}
%The Hausdorff distance between the over-approximative linear combination of the exact affine solutions and of the outer-approximation of the affine solutions can be bounded by \eqref{eq:ecomb}, i.e.,
%%
%\begin{equation*}
%	\dH{\Sover{}, \Zover{}} \leq \sqrt{\gens{}_h + \widehat{\gens{}}_p + \widehat{\gens{}}_p^{\prime}} \,
%		\norm{[G_h^{(-)}~\widehat{G}_p^{(-)}~\widehat{G}_p^{\prime}]}_2 ,
%\end{equation*}
%%
%where the individual terms are defined using \eqref{eq:def_HP}, \eqref{eq:def_overPu_init}, \eqref{eq:def_overPu_k}, and by $G_h^{(-)} := (e^{A\Delta t_k} - I) G_h$, $\widehat{G}_p^{(-)} := (e^{A\Delta t_k} - I) \widehat{G}_p$.
%\end{lemma}
%\begin{proof}
%We re-use the previously defined set $\Sover{}$ and shift the interval of $\lambda$ to $[-1,1]$ to obtain
%%
%\begin{align*}
%	\Sover{} &= \bigg\{ 0.5 \big( (I + e^{A\Delta t_k}) (c_h + \widehat{c}_p) + \widehat{c}_p^{\prime} \big) \\
%	&\quad\, + 0.5 \lambda \big( (e^{A\Delta t_k} - I) (c_h + \widehat{c}_p) + \widehat{c}_p^{\prime} \big) \\
%	&\quad\, + \sum_{i=1}^{\gens{}_h} 0.5 G^{(+)}_{h(\cdot,i)} \varphi_i + \sum_{i=1}^{\widehat{\gens{}}_p} 0.5 \widehat{G}^{(+)}_{p(\cdot,i)} \chi_i
%		+ \sum_{i=1}^{\widehat{\gens{}}_p^{\prime}} 0.5 \widehat{G}^{\prime}_{p(\cdot,i)} \chi_i^{\prime} \\
%	&\quad\, + \sum_{i=1}^{\gens{}_h} 0.5 G^{(-)}_{h(\cdot,i)} \varphi_i \lambda + \sum_{i=1}^{\widehat{\gens{}}_p} 0.5 \widehat{G}^{(-)}_{p(\cdot,i)} \chi_i \lambda \\
%	&\quad\, + \sum_{i=1}^{\widehat{\gens{}}_p^{\prime}} 0.5 \widehat{G}^{\prime}_{p(\cdot,i)} \chi_i^{\prime} \lambda \, \bigg| \,
%		\varphi_i, \chi_i, \chi_i^{\prime}, \lambda \in [-1,1] \bigg\} ,
%\end{align*}
%%
%where we define $G_h^{(+)} := (e^{A\Delta t_k} + I) G_h$, $G_h^{(-)} := (e^{A\Delta t_k} - I) G_h$ (analogously for $\widehat{G}_p$).
%Additionally, we simplify the above expression by a concatenation of generator matrices $G := [G_h^{(-)}~\widehat{G}_p^{(-)}~\widehat{G}_p^{\prime}]$ and by concatenating all corresponding factors $\varphi_i, \chi_i$, and $\chi_i^{\prime}$ to $\psi_i$ where $i \in \{1, ..., \gens{}\}, \gens{} := \gens{}_h + \widehat{\gens{}}_p + \widehat{\gens{}}_p^{\prime}$.
%In order to represent this exact linear combination $\Sover{}$ as a zonotope, we have to substitute the bilinear factors $\psi_i \lambda$ in the last terms by additional linear factors $\omega_i \in [-1,1]$, which results in \eqref{eq:zonoLinComb}, i.e., the outer-approximation $\Zover{}$ of the exact linear combination $\Sover{}$.
%Due to the obvious containment $\Sover{} \subseteq \Zover{}$, the formula \eqref{eq:dH} simplifies to
%%
%\begin{equation} \label{eq:dH_EoverE}
%	\dH{\Sover{},\Zover{}}
%	= \max_{\widehat{z} \in \Zover{}} \min_{\widehat{s} \in \Sover{}} \norm{\widehat{z} - \widehat{s}}_2 ,
%\end{equation}
%%
%for which we compute an upper bound by using identical factors before and after conversion, namely,
%%
%\begin{equation*}
%	\widehat{\lambda} := \lambda, \quad
%	\widehat{\varphi}_i := \varphi_i, \quad
%	\widehat{\chi}_i := \chi_i, \quad
%	\widehat{\chi}_i^{\prime} := \chi_i^{\prime}, \quad
%	\widehat{\psi}_i := \psi_i.
%\end{equation*}
%%
%Consequently, all terms but one cancel out and we obtain
%%
%\begin{align*}
%	\max_{\widehat{z} \in \Zover{}} \min_{\widehat{s} \in \Sover{}} \norm{\widehat{z} - \widehat{s}}_2
%	&\leq \max_{\substack{\omega_i \in [-1,1] \\ \psi_i \in [-1,1] \\ \lambda \in [-1,1]} } 0.5 \norm{ \sum_{i=1}^{\gens{}} G_{(\cdot,i)} (\omega_i - \psi_i \lambda) }_2 \\
%	&\leq \max_{\substack{\Omega \in [-\vecones{},\vecones{}] \\ \Psi \in [-\vecones{},\vecones{}] \\ \lambda \in [-1,1]}}
%		0.5 \norm{ G }_2 \norm{ (\Omega - \Psi \lambda) }_2
%\end{align*}
%%
%writing matrices instead of vectors.
%Due to the convexity \rmk{not entirely true!} of the objective function, we know that the maximizing values of $\Omega, \Psi$, and $\lambda$ have to be on the boundary of their respective domains, hence the maximization is subject to
%%
%\begin{equation*}
%	\forall i \in \{1,...,\gens{}\}: \omega^2_i = 1, \psi^2_i = 1, \quad \text{and} \quad \lambda^2 = 1 .
%\end{equation*}
%%
%We square and expand to obtain
%%
%\begin{align*}
%	&\max_{\substack{\Omega \in [-\vecones{},\vecones{}] \\ \Psi \in [-\vecones{},\vecones{}] \\ \lambda \in [-1,1]} }
%		\norm{ \Omega - \Psi \lambda }^2_2
%	=\max_{\substack{\Omega \in [-\vecones{},\vecones{}] \\ \Psi \in [-\vecones{},\vecones{}] \\ \lambda \in [-1,1]} }
%		\underbrace{\Omega^2}_{= \, \gens{}} + \underbrace{\Psi^2 \lambda^2}_{= \, \gens{}}
%		- \underbrace{2 \lambda \Omega^\top \Psi}_{\in \, [-2\gens{},2\gens{}]} \\
%	&\; \Rightarrow \;
%	\max_{\substack{\Omega \in [-\vecones{},\vecones{}] \\ \Psi \in [-\vecones{},\vecones{}] \\ \lambda \in [-1,1]} }
%		\norm{ \Omega - \Psi \lambda }_2
%	\leq 2 \sqrt{\gens{}} .
%\end{align*}
%%
%Consequently, the error is
%%
%\begin{equation*}
%	\dH{\Sover{},\Zover{}}
%	\leq 0.5 \norm{ G }_2 \, \max_{\substack{\Omega \in [-\vecones{},\vecones{}] \\ \Psi \in [-\vecones{},\vecones{}] \\ \lambda \in [-1,1]}}
%		\norm{ \Omega - \Psi \lambda }_2
%	%= 0.5 \norm{ G }_2 2 \sqrt{\gens{}}
%	= \sqrt{\gens{}} \norm{G}_2 .
%\end{equation*}
%%One may revert to either one of the upper bounds
%%%
%%\begin{equation*}
%%	\norm{G^{(-)}}_2 \leq \sqrt{\norm{G^{(-)}}_1 \norm{G^{(-)}}_\infty} \quad \text{or} \quad
%%	\norm{G^{(-)}}_2 \leq \norm{G^{(-)}}_F \, ,
%%\end{equation*}
%%%
%%with $\norm{\cdot}_F$ denoting the Frobenius norm.
%\end{proof}


% --- proof error affine solution with overPu in appendix





% --- limit behavior of error constant input solution in IV-C

%\begin{lemma} \label{lmm:eaccustep_lim}
%For the error $\eaccustep{k}$ in \eqref{eq:eaccustep}, we have
%\begin{equation*}
%	\lim_{\Delta t_k \to 0} \eaccustep{k} = 0
%	\quad \text{and} \quad
%	\eaccustep{k} \sim \bigO{ \Delta t_k^{\tayl{}+2} }.
%\end{equation*}
%\end{lemma}
%%
%\begin{proof}
%According to \eqref{eq:eaccustep} we have
%\begin{equation*}
%	\eaccustep{k} = 2 \errOp{ \zono{ \matzeros{}, e^{At_k} \widehat{G}_p^{\prime} } }
%\end{equation*}
%where $\widehat{G}_p^{\prime}$ is given by the term $\E{k} \Delta t_k \uTrans{}$.
%By \lmmref{lmm:E_lim}, we yield both the limit value 0 and the asymptotic behavior $\bigO{\eaccustep{k}} = \Delta t_k^{\tayl{k}+2}$.
%\end{proof}

% --- limit behavior of error constant input solution





% --- limit behavior of ehom in IV-C

%\begin{lemma} \label{lmm:ehom_lim}
%For the error $\ehom{k}$ in \eqref{eq:ehom}, we have
%\begin{equation*}
%	\lim_{\Delta t_k \to 0} \ehom{k} = 0 \quad \text{and} \quad \ehom{k} \sim \bigO{ \Delta t_k } .
%\end{equation*}
%\end{lemma}
%\begin{proof}
%We examine the two parts of $\ehom{k} = \ecomb{k} + \eC{k}$ separately, where we begin with $\ecomb{k}$:
%%
%\begin{align*}
%	&\lim_{\Delta t_k \to 0} \ecomb{k} \\
%	\overset{\eqref{eq:ecomb}}&{=} \lim_{\Delta t_k \to 0}
%		\sqrt{\gens{}_h + \widehat{\gens{}}_p + \widehat{\gens{}}_p^{\prime}} \, \norm{[G_h^{(-)}~\widehat{G}_p^{(-)}~\widehat{G}_p^{\prime}]}_2 \\
%	&= \lim_{\Delta t_k \to 0}
%		\sqrt{\gens{}} \, \norm{[(e^{A\Delta t_k} - I) G_h~(e^{A\Delta t_k} - I) \widehat{G}_p~\widehat{G}_p^{\prime}]}_2 \\
%	&= \sqrt{\gens{}} \, \norm{[(e^{\matzeros{}} - I) G_h~(e^{\matzeros{}} - I) \widehat{G}_p~\widehat{G}_p^{\prime}]}_2 \\
%	&= \sqrt{\gens{}} \, \norm{[\matzeros{}~\matzeros{}~\matzeros{}]}_2 = 0
%\end{align*}
%%
%using $\gens{} = \gens{}_h + \widehat{\gens{}}_p + \widehat{\gens{}}_p^{\prime}$ and the fact that $\lim_{\Delta t_k \to 0} \overPu{\Delta t_k} = \matzeros{}$ according to \eqref{eq:overPu_init}.
%To analyze the asymptotic behavior, it suffices to look at the individual generator matrices as the factor $\gens{}$ and the 2-norm are only linear scalings:
%Since $G_h$ and $\widehat{G}_p$ do not depend on $\Delta t_k$, $\widehat{G}_p^{\prime} = \E{k} \Delta t_k \uTrans{}$, and $(e^{A\Delta t_k} - I) \sim \bigO{\Delta t_k}$, we have
%%
%\begin{align*}
%	&(e^{A\Delta t_k} - I) G_h \sim \bigO{ \Delta t_k } \\
%	&(e^{A\Delta t_k} - I) \widehat{G}_p \sim \bigO{ \Delta t_k } \\
%	&\widehat{G}_p^{\prime} = \E{k} \Delta t_k \uTrans{} \overset{\text{\lmmref{lmm:E_lim}}}{\sim} \bigO{ \Delta t_k^{\tayl{k}+2} } .
%\end{align*}
%%
%Consequently, we obtain
%\begin{equation*}
%	\ecomb{k} \sim \bigO{ \Delta t_k } .
%\end{equation*}
%%
%For $\eC{k}$, we have
%\begin{align*}
%	&\lim_{\Delta t_k \to 0} \mathcal{I}_i(\Delta t_k) = \mathcal{I}_i(0) = \big[\big( i^{\frac{-i}{i-1}} - i^{\frac{-1}{i-1}} \big) 0^i,0\big] = 0 , \\
%	&\lim_{\Delta t_k \to 0} \Fx{k} \overset{\eqref{eq:Fx}}{=} \bigoplus_{i=2}^{\tayl{k}} \mathcal{I}_i(0) \, \frac{A^i}{i!} \oplus \Ezero{k} = \matzeros{} , \\
%	&\lim_{\Delta t_k \to 0} \Fu{k} \overset{\eqref{eq:Fu}}{=} \bigoplus_{i=2}^{\tayl{k}+1} \mathcal{I}_i(0) \, \frac{A^i}{i!} \oplus \Ezero{k} 0 = \matzeros{} ,
%\end{align*}
%which entails
%\begin{equation*}
%	\lim_{\Delta t_k \to 0} \eC{k}
%	= 2 ( \errOp{ \Fxzero{} \HPtp{t_k} } + \errOp{ \Fuzero{} \uTrans{} } ) = 0	.
%\end{equation*}
%%
%Moreover, we have $\mathcal{I}_i(\Delta t_k) \sim \bigO{ \Delta t_k^2 }$ as the minimal index is $i=2$, so that we obtain in combination with \lmmref{lmm:E_lim}
%\begin{equation*}
%	\eC{k} \sim \bigO{ \Delta t_k^2 } .
%\end{equation*}
%Since $\ehom{k} = \ecomb{k} + \eC{k}$, it is then straightforward to obtain the limit and asymptotic behavior for $\ehom{k}$.
%\end{proof}

% --- limit behavior of ehom





% --- error time-interval homogeneous solution

%Let us introduce three lemmas for bounding the Hausdorff distance in special cases.
%%
%\begin{lemma} \label{lmm:dH_epi}
%Let $a,b: \mathcal{I} \subset \R{} \to \R{n}$ be two functions and $\S{} = [l,u] \subset \R{n}$ an interval so that $\forall t: a(t) \in b(t) \oplus \S{}$ holds.
%Then,
%%
%\begin{equation*}
%	\dH{a(t),b(t)} \leq \errOp{\S{}} .
%\end{equation*}
%% forall t not necessary, right?
%\end{lemma}
%%
%\begin{proof}
%We reformulate $\forall t: a(t) \in b(t) \oplus \S{}$ to obtain the element-wise inequalities $\forall i \in \{1,...,n\}$:
%%
%\begin{alignat*}{4}
%	&						&&\forall t: b_i(t) + l_i	&&\leq a_i(t)	&&\leq b_i(t) + u_i \\
%	&\Leftrightarrow \;\;	&&\forall t: -a_i(t) + l_i 	&&\leq -b_i(t)	&&\leq -a_i(t) + u_i \\
%	&\Leftrightarrow \;\;	&&\forall t: a_i(t) - u_i	&&\leq b_i(t)	&&\leq a_i(t) - l_i .
%\end{alignat*}
%%
%Using $\mathcal{S}' = [-u,-l] \subset \R{n}$, the last line is equivalent to $\forall t: b(t) \in a(t) \oplus \mathcal{S}'$.
%We over-approximate $\S{}$ and $\mathcal{S}'$ by a symmetric interval $\Sover{} = [\min(l,-u),\max(u,-l)] \subset \R{n}$ where the $\min$- and $\max$-operations are evaluated elementwise.
%\rmk{fixed t results in over-approximation}
%Using both directions of containment for \eqref{eq:dHball}, we obtain
%%
%\begin{equation*}
%	\dH{a(t),b(t)} \leq \rad(\Sover{}) \overset{\eqref{eq:errOp}}{=} \errOp{\S{}} ,
%\end{equation*}
%%
%which yields the claim.
%\end{proof}
%
%\begin{lemma} \label{lmm:dH_2err}
%The premises $\dH{\S{1},\S{2}} \leq \rad(\S{3}) = \varepsilon$ and \linebreak $\S{1} \subseteq \S{2} \oplus \S{3}$ imply $\dH{\S{1},\S{2} \oplus \S{3}} \leq 2\rad(\S{3})$.
%\end{lemma}
%\begin{proof}
%By \eqref{eq:dHball}, we have $\S{2} \subseteq \S{1} \oplus \B{\varepsilon}$.
%Adding $\S{3}$ to both sides yields $\S{2} \oplus \S{3} \subseteq \S{1} \oplus \B{2 \varepsilon}$.
%Combining this result with $\S{1} \subseteq \S{2} \oplus \S{3} \subseteq \S{2} \oplus \S{3} \oplus \B{2 \varepsilon}$ yields the claim.
%\end{proof}
%
%As mentioned in the main body, the proof of \propref{prop:eps_affine} consists of several parts, which we split into lemmata to enhance the readability.
%First, we account for the deviation between the linear interpolation of corresponding points in $\HPtp{t_k}$ and $\HPtp{t_{k+1}}$ and the true trajectories between those two sets.
%
%\begin{lemma} \label{lmm:eps_affine_1}
%The Hausdorff distance between the exact time-interval solution for the affine dynamics and the enlarged exact linear combination is given by second term in the error \eqref{eq:ehom}, i.e.,
%%
%\begin{equation*}
%	\dH{ \HPti{\tau_k},\linCombOp{\HPtp{t_k},\HPtp{t_{k+1}}} \oplus \C{} } \leq 2 \errOp{\C{}}
%\end{equation*}
%%
%with $\tau_k \in [t_k,t_k+\Delta t_k]$.
%\end{lemma}
%\begin{proof}
%For the pointwise solution of the affine dynamics $x^*(t) = x^h(t) + x^u(t)$ composed of the homogeneous solution $x^h(t)$ and the particular solution $x^u(t)$ due to the input vector~$\uTrans{}$, we have \cite[Eq.~(3.10)]{Althoff2010a}
%%
%\begin{align}
%	&x^h(t) \in \tilde{x}^h(t) \oplus \Fx{k} x^*(t_k), \label{eq:affine_h} \\
%	&x^u(t) \in \tilde{x}^u(t) \oplus \Fu{k} \uTrans{} \label{eq:affine_u} \\
%	&\text{with} \; \tilde{x}^h(t) := x^*(t_k) + \frac{t}{\Delta t_k} \big( e^{A \Delta t_k} x^*(t_k) - x^*(t_k) \big) \nonumber \\
%	&\text{and} \; \tilde{x}^u(t) := \matzeros{} + \frac{t}{\Delta t_k} \big( x^u(\Delta t_k) - \matzeros{} \big)  \nonumber
%\end{align}
%%
%for $t \in [t_k,t_k+\Delta t_k]$, which is shown in \figref{fig:affine}.
%%
%\begin{figure}[th]
%\centering
%\input{./figures/affine.tikz}
%\caption{Time interval $t \in [t_k, t_k + \Delta t_k]$: Enclosure of the trajectories $x^h(t)$ and $x^u(t)$ (in blue) by a linear interpolation from the corresponding start to end points, enlarged by sets accounting for the curvature.}
%\label{fig:affine}
%\end{figure}
%
%By applying \lmmref{lmm:dH_epi} to \eqref{eq:affine_h} and \eqref{eq:affine_u}, we obtain 
%\begin{align*}
%	\dH{x^h(t),\tilde{x}^h(t)} &\leq \errOp{\Fx{k} x^*(t_k)} \\
%	\dH{x^u(t),\tilde{x}^u(t)} &\leq \errOp{\Fu{k} \uTrans{}} .
%\end{align*}
%%
%The subsequent application of \lmmref{lmm:dH_2err} yields
%%
%\begin{align*}
%	&\dH{x^h(t),\tilde{x}^h(t) + \Fx{k} x^*(t_k)} \\
%	&\qquad \leq 2 \errOp{\Fx{k} x^*(t_k)} ,
%\end{align*}
%%
%and by extending the first measurement to sets, we obtain $2 \errOp{ \Fx{k} \HPtp{t_k} }$.
%Analogously, we yield
%\begin{equation*}
%	\dH{x^u(t),\tilde{x}^u(t) + \Fu{k} \uTrans{}} \leq 2 \errOp{\Fu{k} \uTrans{}} .
%\end{equation*}
%%
%Their addition then results in $2\errOp{\C{}}$, which yields the claim.
%\end{proof}

% --- error time-interval homogeneous solution






% --- proof for inner-approximation of time-interval homogeneous solution

%\begin{lemma} \label{lmm:eps_affine_1}
%The Hausdorff distance between the exact time-interval solution of the affine dynamics
%%
%\begin{align*}
%	\HPti{\tau_k} &= \big\{ e^{At} x(t_k) + A^{-1}(e^{A (t - t_k)} - I) \uTrans{} ~ \big| \\
%		&\qquad \quad t \in \tau_k, x(t_k) \in \HPtp{t_k} \big\}
%\end{align*}
%%
%and the outer-approximation
%%
%\begin{align*}
%	\overHPti{\tau_k} = \linCombOp{\HPtp{t_k},\HPtp{t_{k+1}}} \oplus \C{}
%\end{align*}
%%
%with $\C{}$ as defined in \lineref{alg:standard:C} of \algref{alg:standard}, can be bounded by
%%
%\begin{align*}
%	\dH{ \HPti{\tau_k}, \linCombOp{\HPtp{t_k},\HPtp{t_{k+1}}} \oplus \C{} }
%	\leq 2 \errOp{\C{}} .
%\end{align*}
%\end{lemma}
%%
%\begin{proof}
%Using a pointwise perspective, it holds that
%%
%\begin{equation} \label{eq:containment_1}
%	\forall t \in \tau_k: x^a(t) \in \tilde{x}^a(t) \oplus \C{}
%\end{equation}
%%
%where $x^a(t)$ denotes the true affine solution trajectory and $\tilde{x}^a(t)$ the linear interpolation.
%Using $\C{} = [l,u]$, we reformulate \eqref{eq:containment_1} to obtain the element-wise inequalities $\forall i \in \{1,...,n\}$:
%%
%\begin{alignat*}{4}
%	&						&&\forall t: \tilde{x}^a_i(t) + l_i		&&\leq x^a_i(t)				&&\leq \tilde{x}^a_i(t) + u_i \\
%	&\Leftrightarrow \;\;	&&\forall t: -x^a_i(t) + l_i			&&\leq -\tilde{x}^a_i(t)	&&\leq -x^a_i(t) + u_i \\
%	&\Leftrightarrow \;\;	&&\forall t: x^a_i(t) - u_i				&&\leq \tilde{x}^a_i(t)		&&\leq x^a_i(t) - l_i .
%\end{alignat*}
%%
%Defining $\C{}' = [-u,-l] \subset \R{n}$, the last line is equivalent to
%%
%\begin{equation} \label{eq:containment_2}
%	\forall t: \tilde{x}^a(t) \in x^a(t) \oplus \C{}'
%	\, \Leftrightarrow \,
%	\forall t: x^a(t) \ominus \C{}' \in \tilde{x}^a(t)
%\end{equation}
%%
%by the definition of the Minkowski difference \eqref{eq:defMinDiff}.
%Let us over-approximate $\C{}$ and $\C{}'$ by a symmetric interval $\widehat{\mathcal{C}} = [\min(l,-u),\max(u,-l)] \subset \R{n}$ where the $\min$- and $\max$-operations are evaluated element-wise.
%Then, we extend \eqref{eq:containment_1} and \eqref{eq:containment_2} to sets, yielding two containments
%%
%\begin{align*}
%	\HPtp{\tau_k} &\subseteq \linCombOp{\HPtp{t_k},\HPtp{t_{k+1}}} \oplus \widehat{\mathcal{C}} , \\
%	\HPtp{\tau_k} &\supseteq \linCombOp{\HPtp{t_k},\HPtp{t_{k+1}}} \ominus \widehat{\mathcal{C}} .
%\end{align*}
%%
%This immediately entails
%%
%\begin{equation*}
%	\dH{ \HPtp{\tau_k}, \linCombOp{\HPtp{t_k},\HPtp{t_{k+1}}} \oplus \C{} } \leq 2 \errOp{ \C{} } ,
%\end{equation*}
%%
%where we exploit that $\errOp{\widehat{C}} = \errOp{\C{}}$ by \eqref{eq:errOp}.
%\end{proof}

% --- proof for inner-approximation of time-interval homogeneous solution




% --- proof triangle inequality for affine error

%\noindent
%\textit{Proof of \propref{prop:eps_affine}:}
%The error for the affine dynamics solution can be bounded using the triangle inequality:
%%
%\begin{align*}
%	&\dH{ \HPti{\tau_k}, \linCombOpZ{\HPtp{t_k},\HPtp{t_{k+1}}} \oplus \C{} } \\
%	&\qquad \leq \dH{ \HPti{\tau_k}, \linCombOp{\HPtp{t_k},\HPtp{t_{k+1}}} \oplus \C{} } \\
%	&\qquad \quad + d_H \big( \linCombOp{\HPtp{t_k},\HPtp{t_{k+1}}} \oplus \C{}, \\
%	&\qquad \qquad \qquad \, \linCombOpZ{\HPtp{t_k},\HPtp{t_{k+1}}} \oplus \C{} \big) .
%\end{align*}
%%
%The two Hausdorff distances on the right-hand side are given by \lmmsref{lmm:eps_affine_1}{lmm:eps_affine_2}, which we add to obtain the bound in \eqref{eq:ehom}.
%$\hfill \square$

% --- proof triangle inequality for affine error

